Partial Entropy production of active particles with hidden states in potentials

Partially observed stochastic systems can appear (almost) time-reversal symmetric while in fact operating far from equilibrium. The present work extends the perturbative framework introduced in [Phys. Rev. Lett. 136, 198302 (2026)] to calculate in a generic confining potential the partial entropy production, which quantifies the time-reversal asymmetry of a generic active particle with hidden self-propulsion. Focusing on the harmonic case, we apply our framework to reproduce an exact result for the partial entropy production rate of an active Ornstein-Uhlenbeck particle and to derive the partial entropy production rate of a run-and-tumble particle.

==> macros.tex <==


\newcommand{\gpcomment}[1]{\textcolor{orange}{[GP: #1]}}


\makeatletter
\DeclareFontFamily{OMX}{MnSymbolE}{}
\DeclareSymbolFont{MnLargeSymbols}{OMX}{MnSymbolE}{m}{n}
\SetSymbolFont{MnLargeSymbols}{bold}{OMX}{MnSymbolE}{b}{n}
\DeclareFontShape{OMX}{MnSymbolE}{m}{n}{
    <-6>  MnSymbolE5
   <6-7>  MnSymbolE6
   <7-8>  MnSymbolE7
   <8-9>  MnSymbolE8
   <9-10> MnSymbolE9
  <10-12> MnSymbolE10
  <12->   MnSymbolE12
}{}
\DeclareFontShape{OMX}{MnSymbolE}{b}{n}{
    <-6>  MnSymbolE-Bold5
   <6-7>  MnSymbolE-Bold6
   <7-8>  MnSymbolE-Bold7
   <8-9>  MnSymbolE-Bold8
   <9-10> MnSymbolE-Bold9
  <10-12> MnSymbolE-Bold10
  <12->   MnSymbolE-Bold12
}{}

\let\llangle\@undefined
\let\rrangle\@undefined
\DeclareMathDelimiter{\llangle}{\mathopen}
                     {MnLargeSymbols}{'164}{MnLargeSymbols}{'164}
\DeclareMathDelimiter{\rrangle}{\mathclose}
                     {MnLargeSymbols}{'171}{MnLargeSymbols}{'171}
\makeatother





\newcommand{\plaind}{\mathrm{d}}
\newcommand{\dint}[1]{\mathchoice{\!\plaind#1\,}{\!\plaind#1\,}{\!\plaind#1\,}{\!\plaind#1\,}}
\newcommand{\ddint}[1]{\ddintx{#1}{d}}
\newcommand{\dTWOint}[1]{\ddintx{#1}{2}}
\newcommand{\ddintx}[2]{\mathchoice{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}}
\newcommand{\ddMOneint}[1]{\mathchoice{\!\plaind^{d-1}#1\,}{\!\plaind^{d-1}#1\,}{\!\plaind^{d-1}#1\,}{\!\plaind^{d-1}#1\,}}
\newcommand{\Xddint}[2]{\mathchoice{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}{\!\plaind^{#2}#1\,}}
\newcommand{\dbar}{\text{\dj}}
\newcommand{\deltabar}{\delta\mkern-6mu\mathchar'26}
\newcommand{\dintbar}[1]{\mathchoice{\!\dbar#1\,}{\!\dbar#1\,}{\!\dbar#1\,}{\!\dbar#1\,}}
\newcommand{\ddintbar}[1]{\mathchoice{\!\dbar^d#1\,}{\!\dbar^d#1\,}{\!\dbar^d#1\,}{\!\dbar^d#1\,}}
\newcommand{\dTWOintbar}[1]{\mathchoice{\!\dbar^2#1\,}{\!\dbar^2#1\,}{\!\dbar^2#1\,}{\!\dbar^2#1\,}}
\newcommand{\ddMOneintbar}[1]{\mathchoice{\!\dbar^{d-1}#1\,}{\!\dbar^{d-1}#1\,}{\!\dbar^{d-1}#1\,}{\!\dbar^{d-1}#1\,}}
\newcommand{\Dint}[1]{\!\!\mathcal{D}#1\,}
\DeclareFontFamily{U}{wncy}{}
\DeclareFontShape{U}{wncy}{m}{n}{<->wncyr10}{}
\DeclareSymbolFont{mcy}{U}{wncy}{m}{n}
\DeclareMathSymbol{\sha}{\mathord}{mcy}{"58}


\newcommand{\MCLineVsMathEnv}[2]{\mathchoice{#1}{#2}{#2}{#2}}
\newcommand{\dX}[1]{\plaind #1}
\newcommand{\dx}{\dX{x}}
\newcommand{\ds}{\dX{s}}
\newcommand{\dt}{\dX{t}}
\newcommand{\ddX}[1]{\MCLineVsMathEnv{\frac{\plaind}{\plaind #1}}{\plaind/\plaind #1}}
\newcommand{\ddt}{\ddX{t}}
\newcommand{\ddx}{\ddX{x}}
\newcommand{\dds}{\ddX{s}}
\newcommand{\ddXX}[2]{\MCLineVsMathEnv{\frac{\plaind #1}{\plaind #2}}{\plaind #1/\plaind #2}}
\newcommand{\ddtX}[1]{\ddXX{#1}{t}}
\newcommand{\ddxX}[1]{\ddXX{#1}{x}}
\newcommand{\ddsX}[1]{\ddXX{#1}{s}}
\newcommand{\ppX}[1]{\MCLineVsMathEnv{\frac{\partial}{\partial #1}}{\partial/\partial #1}}
\newcommand{\ppx}{\ppX{x}}
\newcommand{\ppt}{\ppX{t}}
\newcommand{\ppXX}[2]{\MCLineVsMathEnv{\frac{\partial #1}{\partial #2}}{\partial #1/\partial #2}}
\newcommand{\pptX}[1]{\ppXX{#1}{t}}
\newcommand{\ppxX}[1]{\ppXX{#1}{x}}
\newcommand{\ppsX}[1]{\ppXX{#1}{s}}

\usepackage{dsfont}
\newcommand{\OLDgpset}[1]{\mathbb{#1}}
\newcommand{\gpset}[1]{\mathds{#1}}

\newcommand{\canetset}[1]{{\mathchoice {\hbox{$\sf\textstyle #1\kern-0.4em #1$}}
{\hbox{$\sf\textstyle #1\kern-0.4em #1$}}
{\hbox{$\sf\scriptstyle #1\kern-0.3em #1$}}
{\hbox{$\sf\scriptscriptstyle #1\kern-0.2em #1$}}}}

\newcommand{\Nset}{\gpset{N}}
\newcommand{\Pset}{\gpset{P}}
\newcommand{\Zset}{\gpset{Z}}
\newcommand{\Qset}{\gpset{Q}}
\newcommand{\Rset}{\gpset{R}}
\newcommand{\Cset}{\gpset{C}}
\newcommand{\Sset}{\gpset{S}}
\newcommand{\Wset}{\gpset{W}}





\def\nbZ{{\mathchoice {\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\textstyle Z\kern-0.4em Z$}}
{\hbox{$\sf\scriptstyle Z\kern-0.3em Z$}}
{\hbox{$\sf\scriptscriptstyle Z\kern-0.2em Z$}}}}

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bj}{\mathbf{j}}
\newcommand{\bk}{\mathbf{k}}
\newcommand{\bl}{\mathbf{l}}
\newcommand{\bx}{\mathbf{x}}
\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}


\newcommand{\gpvec}[1]{\mathbf{#1}}


\newcommand{\zerovec}{\gpvec{0}}
\newcommand{\nullvec}{\zerovec}
\newcommand{\avec}{\gpvec{a}}
\newcommand{\bvec}{\gpvec{b}}
\newcommand{\cvec}{\gpvec{c}}
\newcommand{\dvec}{\gpvec{d}}
\newcommand{\evec}{\gpvec{e}}
\newcommand{\fvec}{\gpvec{f}}
\newcommand{\gvec}{\gpvec{g}}
\newcommand{\ivec}{\gpvec{i}}
\newcommand{\jvec}{\gpvec{j}}
\newcommand{\kvec}{\gpvec{k}}
\newcommand{\ellvec}{\gpvec{\ell}}
\newcommand{\mvec}{\gpvec{m}}
\newcommand{\nvec}{\gpvec{n}}
\newcommand{\pvec}{\gpvec{p}}
\newcommand{\qvec}{\gpvec{q}}
\newcommand{\rvec}{\gpvec{r}}
\newcommand{\svec}{\gpvec{s}}
\newcommand{\uvec}{\gpvec{u}}
\newcommand{\vvec}{\gpvec{v}}
\newcommand{\wvec}{\gpvec{w}}
\newcommand{\xvec}{\gpvec{x}}
\newcommand{\yvec}{\gpvec{y}}
\newcommand{\zvec}{\gpvec{z}}

\newcommand{\Avec}{\gpvec{A}}
\newcommand{\Bvec}{\gpvec{B}}
\newcommand{\Cvec}{\gpvec{C}}
\newcommand{\Evec}{\gpvec{E}}
\newcommand{\Fvec}{\gpvec{F}}
\newcommand{\Hvec}{\gpvec{H}}
\newcommand{\Ivec}{\gpvec{I}}
\newcommand{\Jvec}{\gpvec{J}}
\newcommand{\Kvec}{\gpvec{K}}
\newcommand{\Mvec}{\gpvec{M}}
\newcommand{\Nvec}{\gpvec{N}}
\newcommand{\Pvec}{\gpvec{P}}
\newcommand{\Qvec}{\gpvec{Q}}
\newcommand{\Rvec}{\gpvec{R}}
\newcommand{\Svec}{\gpvec{S}}
\newcommand{\Uvec}{\gpvec{U}}
\newcommand{\Vvec}{\gpvec{V}}
\newcommand{\Wvec}{\gpvec{W}}
\newcommand{\Xvec}{\gpvec{X}}
\newcommand{\Yvec}{\gpvec{Y}}
\newcommand{\Zvec}{\gpvec{Z}}

\newcommand{\alphavec}{\bm{\alpha}}
\newcommand{\betavec}{\bm{\beta}}
\newcommand{\deltavec}{\bm{\delta}}
\newcommand{\gammavec}{\bm{\gamma}}
\newcommand{\epsilonvec}{\bm{\epsilon}}
\newcommand{\muvec}{\bm{\mu}}
\newcommand{\nuvec}{\bm{\nu}}
\newcommand{\phivec}{\bm{\phi}}
\newcommand{\varphivec}{\bm{\varphi}}
\newcommand{\xivec}{\bm{\xi}}
\newcommand{\zetavec}{\bm{\zeta}}


\newcommand{\transpose}{\mathsf{T}}
\newcommand{\ident}{\mathds{1}}
\newcommand{\unity}{\ident}
\newcommand{\Trace}{\operatorname{Tr}}

\newcommand*\laplace{\mathop{}\!\mathbin\bigtriangleup}


\newcommand{\erf}{\operatorname{erf}}
\newcommand{\erfc}{\operatorname{erfc}}

\newcommand{\BC}{\mathcal{B}}
\newcommand{\CC}{\mathcal{C}}
\newcommand{\DC}{\mathcal{D}}
\newcommand{\EC}{\mathcal{E}}
\newcommand{\FC}{\mathcal{F}}
\newcommand{\GC}{\mathcal{G}}
\newcommand{\HC}{\mathcal{H}}
\newcommand{\IC}{\mathcal{I}}
\newcommand{\JC}{\mathcal{J}}
\newcommand{\KC}{\mathcal{K}}
\newcommand{\LC}{\mathcal{L}}
\newcommand{\MC}{\mathcal{M}}
\newcommand{\NC}{\mathcal{N}}
\newcommand{\OC}{\mathcal{O}}
\newcommand{\PC}{\mathcal{P}}
\newcommand{\RC}{\mathcal{P}}
\newcommand{\TC}{\mathcal{T}}
\newcommand{\VC}{\mathcal{V}}
\newcommand{\WC}{\mathcal{W}}
\newcommand{\XC}{\mathcal{X}}
\newcommand{\ZC}{\mathcal{Z}}


\newcommand{\Gtilde}{\tilde{G}}
\newcommand{\GCtilde}{\tilde{\GC}}
\newcommand{\GammaTilde}{\tilde{\Gamma}}

\newcommand{\jtilde}{\tilde{j}}
\newcommand{\mtilde}{\tilde{m}}
\newcommand{\stilde}{\tilde{s}}
\newcommand{\ttilde}{\tilde{t}}
\newcommand{\utilde}{\tilde{u}}
\newcommand{\ytilde}{\tilde{y}}
\newcommand{\Gammatilde}{\tilde{\Gamma}}
\newcommand{\gammatilde}{\tilde{\gamma}}
\newcommand{\phitilde}{\tilde{\phi}}
\newcommand{\chitilde}{\tilde{\chi}}
\newcommand{\adagger}{a^{\dagger}}
\newcommand{\phidagger}{\phi^{\dagger}}
\newcommand{\psitilde}{\tilde{\psi}}
\newcommand{\tautilde}{\tilde{\tau}}
\newcommand{\mutilde}{\tilde{\mu}}


\newcommand{\Ghat}{\hat{G}}
\newcommand{\What}{\hat{W}}
\newcommand{\Gammahat}{\hat{\Gamma}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\jhat}{\hat{j}}

\newcommand{\half}{\mathchoice{\frac{1}{2}}{(1/2)}{\frac{1}{2}}{(1/2)}}
\newcommand{\threehalf}{\mathchoice{\frac{3}{2}}{(3/2)}{\frac{3}{2}}{(3/2)}}
\newcommand{\fourth}{\mathchoice{\frac{1}{4}}{(1/4)}{\frac{1}{4}}{(1/4)}}
\newcommand{\third}{\mathchoice{\frac{1}{3}}{(1/3)}{\frac{1}{3}}{(1/3)}}
\newcommand{\quarter}{\fourth}

\newcommand{\EXP}[1]{\operatorname{exp}\!\Bigg\{#1\Bigg\}}
\newcommand{\Exp}[1]{\operatorname{exp}\left(#1\right)}
\renewcommand{\exp}[1]{\mathchoice
{\mathrm{e}^{#1}}
{\operatorname{exp}(#1)}
{\operatorname{exp}\left(#1\right)}
{\operatorname{exp}\left(#1\right)}}
\newcommand{\exP}{\operatorname{exp}}
\newcommand{\sgn}{\operatorname{sgn}}


\newcommand{\elabel}[1]{\label{eq:#1}}
\newcommand{\eref}[1]{(\ref{eq:#1})}
\newcommand{\Eref}[1]{\mbox{Eq.~(\ref{eq:#1})}}
\newcommand{\Erefs}[1]{\mbox{Eqs.~(\ref{eq:#1})}}

\newcommand{\seclabel}[1]{\label{sec:#1}}
\newcommand{\sref}[1]{\ref{sec:#1}}
\newcommand{\Sref}[1]{Sec.~\ref{sec:#1}}
\newcommand{\Srefs}[1]{Secs.~\ref{sec:#1}}
\newcommand{\ASref}[1]{Appendix~\ref{sec:#1}}
\newcommand{\APref}[1]{\mbox{App.~\ref{sec:#1}}}
\newcommand{\oldSMref}[1]{\mbox{Suppl.~\ref{sec:#1}}}
\newcommand{\SMref}[1]{\mbox{Suppl.~\ref{sec:#1}} \cite{PRRsupplement}}
\newcommand{\SMrefLocal}[1]{Suppl.~\ref{sec:#1}}


\newcommand{\flabel}[1]{\label{fig:#1}}
\newcommand{\fref}[2][]{\ref{fig:#2}#1}
\newcommand{\Frefs}[2][]{Figs.~\ref{fig:#2}#1}
\newcommand{\Fref}[2][]{Fig.~\ref{fig:#2}#1}
\newcommand{\subfref}[2][]{\subref{fig:#2}#1}

\newcommand{\tlabel}[1]{\label{tab:#1}}
\newcommand{\Tref}[1]{Tab.~\ref{tab:#1}}
\newcommand{\tref}[1]{tab.~\ref{tab:#1}}

\newcommand{\latin}[1]{{\it #1}}
\newcommand{\ie}{\latin{i.e.}\@\xspace}
\newcommand{\eg}{\latin{e.g.}\@\xspace}
\newcommand{\cf}{\latin{cf.}\@\xspace}
\newcommand{\etc}{\latin{etc.}\@\xspace}
\newcommand{\viz}{\latin{viz.}\@\xspace}
\newcommand{\etal}{\latin{et~al}.\@\xspace}
\newcommand{\vs}{\latin{vs}.\@\xspace}
\newcommand{\glossarykeyword}[1]{\textcolor{blue}{\bf #1}}
\newcommand{\keyword}[1]{{\bf #1}}
\newcommand{\pname}[1]{\textsc{#1}} 
\newcommand{\eetin}[1]{\emph{#1}}
\newlength \standardfigwidth
\setlength \standardfigwidth{0.66\linewidth}


\DeclareMathAlphabet{\matheub}{U}{eur}{m}{n}
\newcommand{\unitX}[1]{\matheub{#1}}
\newcommand{\Angstrom}{\unitX{\AA}}
\newcommand{\dimof}[1]{\left[#1\right]}
\newcommand{\unitL}{\unitX{L}}
\newcommand{\unitT}{\unitX{T}}
\newcommand{\unitA}{\unitX{A}}
\newcommand{\unitB}{\unitX{B}}
\newcommand{\unitz}{\unitX{z}}



\newcommand{\Adim}{\mathtt{A}}
\newcommand{\Bdim}{\mathtt{B}}
\newcommand{\Cdim}{\mathtt{C}}
\newcommand{\Ldim}{\mathtt{L}}


\newcommand{\V}[1]{\text{Var}\left(#1\right)}
\newcommand{\E}[1]{\text{E}\left[#1\right]}

\newcommand{\renorm}{\mathcal{R}}
\newcommand{\ai}[4]{{\left[\begin{smallmatrix}\textcolor{cyan}{#1}&\textcolor{cyan}{#2}\\\textcolor{orange}{#3}&\textcolor{orange}{#4}\end{smallmatrix}\right]}}
\newcommand{\Gammaai}[4]{\Gamma^{\ai{#1}{#2}{#3}{#4}}}
\newcommand{\Gai}[4]{G^{\ai{#1}{#2}{#3}{#4}}}
\newcommand{\xPs}{P_{\text{surv}}}
\newcommand{\Ps}{P_{\text{s}}}




\usepackage{tikz}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{arrows,shapes,decorations,automata,backgrounds,petri}
\usetikzlibrary{calc}
\usetikzlibrary{patterns}
\usetikzlibrary{decorations.text}

\newcommand\Overline[2][1pt]{
    \begin{tikzpicture}[baseline=(a.base)]
      \node[inner xsep=0pt,inner ysep=1.5pt] (a) {$#2$};
      \draw[line width= #1] (a.north west) -- (a.north east);
    \end{tikzpicture}
    }



\makeatletter
\let\save@mathaccent\mathaccent
\newcommand*\if@single[3]{
  \setbox0\hbox{${\mathaccent"0362{#1}}^H$}
  \setbox2\hbox{${\mathaccent"0362{\kern0pt#1}}^H$}
  \ifdim\ht0=\ht2 #3\else #2\fi
  }
\newcommand*\rel@kern[1]{\kern#1\dimexpr\macc@kerna}
\newcommand*\wideaccent[2]{\@ifnextchar^{{\wide@accent{#1}{#2}{0}}}{\wide@accent{#1}{#2}{1}}}
\newcommand*\wide@accent[3]{\if@single{#2}{\wide@accent@{#1}{#2}{#3}{1}}{\wide@accent@{#1}{#2}{#3}{2}}}
\newcommand*\wide@accent@[4]{
  \begingroup
  \def\mathaccent##1##2{
    \let\mathaccent\save@mathaccent
    \if#42 \let\macc@nucleus\first@char \fi
    \setbox\z@\hbox{$\macc@style{\macc@nucleus}_{}$}
    \setbox\tw@\hbox{$\macc@style{\macc@nucleus}{}_{}$}
    \dimen@\wd\tw@
    \advance\dimen@-\wd\z@
    \divide\dimen@ 3
    \@tempdima\wd\tw@
    \advance\@tempdima-\scriptspace
    \divide\@tempdima 10
    \advance\dimen@-\@tempdima
    \ifdim\dimen@>\z@ \dimen@0pt\fi
    \rel@kern{0.6}\kern-\dimen@
    \if#41
      #1{\rel@kern{-0.6}\kern\dimen@\macc@nucleus\rel@kern{0.4}\kern\dimen@}
      \advance\dimen@0.4\dimexpr\macc@kerna
      \let\final@kern#3
      \ifdim\dimen@<\z@ \let\final@kern1\fi
      \if\final@kern1 \kern-\dimen@\fi
    \else
      #1{\rel@kern{-0.6}\kern\dimen@#2}
    \fi
  }
  \macc@depth\@ne
  \let\math@bgroup\@empty \let\math@egroup\macc@set@skewchar
  \mathsurround\z@ \frozen@everymath{\mathgroup\macc@group\relax}
  \macc@set@skewchar\relax
  \let\mathaccentV\macc@nested@a
  \if#41
    \macc@nested@a\relax111{#2}
  \else
    \def\gobble@till@marker##1\endmarker{}
    \futurelet\first@char\gobble@till@marker#2\endmarker
    \ifcat\noexpand\first@char A\else
      \def\first@char{}
    \fi
    \macc@nested@a\relax111{\first@char}
  \fi
  \endgroup
}
\makeatother

\newcommand\doubleoverline[1]{\overline{\overline{#1}}}

\newcommand\widebar{\wideaccent\overline}
\newcommand\widebarbar{\wideaccent\doubleoverline}


\makeatletter
\newcommand{\spave}[2][]{\@ifempty{#1}{}{\left.}\Overline[1pt]{#2}\@ifempty{#1}{}{\right|_{#1}}}
\newcommand{\thinspave}[2][]{\@ifempty{#1}{}{\left.}\overline{#2}\@ifempty{#1}{}{\right|_{#1}}}
\newcommand{\dave}[2][]{\mathchoice
{\left\llangle #2 \right\rrangle_{#1}}
{\left\llangle #2 \right\rrangle_{#1}}
{\llangle #2\rrangle_{#1}}
{\llangle #2\rrangle_{#1}}}
\newcommand{\ave}[2][]{\mathchoice
{\left\langle #2 \right\rangle_{#1}}
{\left\langle #2 \right\rangle_{#1}}
{\langle #2\rangle_{#1}}
{\langle #2\rangle_{#1}}}
\newcommand{\aveS}[3][]{\mathchoice
{\left\langle #2 \right\rangle_{#1}^{#3}}
{\left\langle #2 \right\rangle_{#1}^{#3}}
{\langle #2\rangle_{#1}^{#3}}
{\langle #2\rangle_{#1}^{#3}}}
\newcommand{\have}[2][]{\@ifempty{#1}{}{\left.}\widehat{#2}\@ifempty{#1}{}{\right|_{#1}}}

\newcommand\doverline[1]{
\tikz[baseline=(nodeAnchor.base)]{
    \node[inner sep=0] (nodeAnchor) {$#1$};
    \draw[line width=0.1ex,line cap=round]
        ($(nodeAnchor.north west)+(0.0em,0.2ex)$)
            --
        ($(nodeAnchor.north east)+(0.0em,0.2ex)$)
        ($(nodeAnchor.north west)+(0.0em,0.5ex)$)
            --
        ($(nodeAnchor.north east)+(0.0em,0.5ex)$)
    ;
}}


\newcommand{\Xbave}[2][]{\@ifempty{#1}{}{\left.}\overline{\overline{#2}}\@ifempty{#1}{}{\right|_{#1}}}
\newcommand{\bave}[2][]{\@ifempty{#1}{}{\left.}\doverline{#2}\@ifempty{#1}{}{\right|_{#1}}}
\makeatother





\newcommand{\Xave}[2][]{\thinspave[#1]{#2}}
\newcommand{\XIave}[2][]{\dave{#2}_{#1}}
\newcommand{\WSTARave}[2][\!*]{\ave[#1]{#2}}
\newcommand{\WSTARaveS}[3][\!*]{\aveS[#1]{#2}{#3}}
\newcommand{\Wave}[2][]{\ave[#1]{#2}}
\newcommand{\WaveS}[3][]{\aveS[#1]{#2}{#3}}



\newcommand{\Pprob}{\mathds{P}}
\newcommand{\PprobX}{\mathds{P}}
\newcommand{\PprobXI}{\mathds{P}}
\newcommand{\PprobXW}{\mathds{P}}
\newcommand{\PprobWSTAR}{\mathds{P}_{\!*}}
\newcommand{\PprobW}{\mathds{P}}

\newcommand{\NormWSTAR}{\NC_{\!*}}



\newcommand{\Psurv}{P_\text{s}}
\newcommand{\cov}[2]{\text{Cov}\left(#1,#2\right)}
\newcommand{\Pext}{P_\text{e}(t)}
\newcommand{\var}[1]{\text{Var}\left( #1 \right)}
\newcommand{\pgf}{f}
\newcommand{\union}{\cup}
\newcommand{\plaint}{\mathrm{t}}
\newcommand{\bra}[1]{\left\langle#1\right|}
\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\braket}[2]{\left\langle#1\middle|#2\right\rangle}
\newcommand{\sandwich}[3]{\left\langle#1\middle|#2\middle|#3\right\rangle}
\newcommand{\creat}{a^\dagger}
\makeatletter
\newcommand{\creatX}[2][]{a^{\@ifempty{#1}{\dagger}{\dagger\,#1}}\@ifempty{#2}{}{(#2)}}
\makeatother
\newcommand{\creatDS}{\tilde{a}}
\makeatletter
\newcommand{\creatDSX}[2][]{\@ifempty{#1}{\creatDS}{\creatDS^{#1}}\@ifempty{#2}{}{(#2)}}
\makeatother
\newcommand{\annih}{a}
\makeatletter
\newcommand{\annihX}[2][]{a\@ifempty{#1}{}{^{#1}}\@ifempty{#2}{}{(#2)}}
\newcommand{\kernel}[1]{K\@ifempty{#1}{}{\,\!\!\left(#1\right)}}
\newcommand{\kernelDeri}[1]{K'\@ifempty{#1}{}{\left(#1\right)}}
\newcommand{\Kmatrix}{\mathsf{K}}
\newcommand{\Okernel}[1]{K\left(#1\right)}
\newcommand{\OkernelDeri}[1]{K'\left(#1\right)}


\newcommand{\tableofappendixcontents}{\@starttoc{toa}}
\newcommand{\l@toact}[2]{\@dottedtocline{1}{1.5em}{5.5em}{#1}{#2}}
\newcommand{\l@toactspace}[2]{\ \hfil}
\makeatother
\newcommand{\tildephi}{\widetilde\phi}
\newcommand{\atilde}{\widetilde{a}}
\newcommand{\tildepsi}{\widetilde{\psi}}
\newcommand{\tildealpha}{\widetilde{\alpha}}

\newcommand{\tilden}{\widetilde{n}}
\newcommand{\ntilde}{\tilden}

\newcommand{\tildeq}{\widetilde{q}}
\newcommand{\qtilde}{\tildeq}

\newcommand{\xdot}{\dot{x}}

\newcommand{\tomega}{\widetilde{\omega}}
\newcommand{\tildebeta}{\widetilde{\beta}}
\newcommand{\tilderho}{\widetilde{\rho}}
\newcommand{\tildenu}{\widetilde{\nu}}
\newcommand{\tildeU}{\widetilde{\mathcal{U}}}
\newcommand{\creatphi}{\phi^\dagger}
\newcommand{\Esref}[1]{Eqs.~(\ref{eq:#1})}
\newcommand{\imag}{\mathring{\imath}}
\newcommand{\commutator}[2]{\left[#1,#2\right]}
\newcommand{\anticommutator}[2]{\left\{#1,#2\right\}_{+}}
\newcommand{\corresponding}{\hat{=}}
\newcommand{\jcomment}[1]{\textcolor{teal}{[JP: #1]}}
\newcommand{\bcomment}[1]{\textcolor{lime}{[BW: #1]}}
\newcommand{\mA}{\mathcal{A}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mG}{\mathcal{G}}
\newcommand{\mJ}{\mathcal{J}}
\newcommand{\mL}{\mathcal{L}}
\newcommand{\mK}{\mathcal{K}}
\newcommand{\mO}{\mathcal{O}}
\newcommand{\mU}{\mathcal{U}}
\newcommand{\Num}{N}
\newcommand{\densfield}{\phi}
\newcommand{\densvec}{\pmb{\phi}}

\newcommand{\fudge}{f}
\newcommand{\massFix}{r}
\newcommand{\Seps}{S_\epsilon}
\newcommand{\identMmOne}{\ident}



\newcommand{\xtmin}{t_\text{min}}
\newcommand{\tmin}{t_1}
\newcommand{\xgtotal}{\mathfrak{g}}
\newcommand{\gtotal}{\hat{g}}
\newcommand{\gbinary}{g}
\newcommand{\Stirling}[2]{\begin{Bmatrix}{#1}\\{#2}\end{Bmatrix}}
\newcommand{\avsh}[2]{V\left(#1,#2\right)}
\newcommand{\xcumavsh}[2]{\pi\left(#1,#2\right)}
\newcommand{\cumavsh}{\Big\langle N(t) \Big| N(T)=0\Big\rangle}

\newcommand{\sdots}{\ifmmode\mathinner{\ldotp\kern-0.2em\ldotp\kern-0.2em\ldotp}\else.\kern-0.13em.\kern-0.13em.\fi}

\newcommand{\bUnity}{\boldsymbol{1}}

\usepackage{xspace}



\newcommand{\xrevision}[2]{\textcolor{red}{#2}}
\newcommand{\revision}[2]{{#2}}
\newcommand{\ijinej}{\substack{i,j\\i\ne j}}
\newcommand{\entropyProduction}{\dot{S}_{\text{int}}}
\newcommand{\entropyProductionDensity}{\dot{\sigma}}
\newcommand{\entropyProductionDensityFourier}{\dot{\hat{\sigma}}}
\newcommand{\entropyProductionDensityTilde}{\dot{\tilde{\sigma}}}
\newcommand{\entropyFlow}{\dot{S}_e}
\newcommand{\Deltar}{{\Delta r}}
\newcommand{\Deltat}{{\Delta t}}
\newcommand{\Deltax}{{\Delta x}}
\newcommand{\Pstate}{P}
\newcommand{\transform}{\mathcal{T}}
\newcommand{\transformTilde}{\tilde{\transform}}


\newcommand{\transMatLin}{\MC}
\newcommand{\transMatNonLin}{\BC}
\newcommand{\PertOp}{\hat{\GC}}
\newcommand{\transMatT}{\hat{\transMatLin}}
\newcommand{\transMatTNonLin}{\hat{\transMatNonLin}}

\newcommand{\Transition}{\WC} 
\newcommand{\TransitionRate}{\mathring{\Transition}}



\newcommand{\EPR}{\dot{S}}
\newcommand{\EPRfull}{\EPR_{x,w}}
\newcommand{\EPRpartW}{\EPR_{w}}
\newcommand{\EPRpartX}{\EPR_{x}}
\newcommand{\SymParity}{\mathcal{P}}
\newcommand{\NotSymParity}{\cancel{\SymParity}}
\newcommand{\SymTime}{\mathcal{T}}
\newcommand{\NotSymTime}{\cancel{\SymTime}}
\newcommand{\SymParityTime}{\mathcal{PT}}

\newcommand{\xpath}{\{x(t)\}}
\newcommand{\Mxpath}{\{-x(t)\}}
\newcommand{\Rxpath}{\{x(T-t)\}}

\newcommand{\wpath}{\{w(t)\}}
\newcommand{\wdpath}{\{w'(t)\}}
\newcommand{\Mwdpath}{\{-w'(t)\}}
\newcommand{\wddpath}{\{w''(t)\}}
\newcommand{\wdddpath}{\{w'''(t)\}}
\newcommand{\Mwpath}{\{-w(t)\}}
\newcommand{\Rwpath}{\{w(T-t)\}}
\newcommand{\Rwdpath}{\{w'(T-t)\}}
\newcommand{\RMwpath}{\{-w(T-t)\}}

\newcommand{\xipath}{\{\xi(t)\}}


\newcommand{\diffw}{D_w}
\newcommand{\resettingRate}{r}
\newcommand{\propagator}[1]{G\!\left(#1\right)}
\newcommand{\propagatorFourier}[1]{\hat{G}\!\left(#1\right)}
\newcommand{\bbar}{\beta}


\makeatletter
\newcommand{\pushright}[1]{\ifmeasuring@#1\else\omit\hfill$\displaystyle#1$\fi\ignorespaces}
\newcommand{\pushleft}[1]{\ifmeasuring@#1\else\omit$\displaystyle#1$\hfill\fi\ignorespaces}
\makeatother

\newcommand{\nlowest}{{n^{\!*}}}
\makeatletter
\newcommand{\corrStar}[1][]{\@ifempty{#1}{}{}\CC\@ifempty{#1}{}{^{(#1)}}}
\makeatother
\newcommand{\gpmatrix}[1]{\bm{\mathsf{#1}}}
\newcommand{\Wmatrix}{\gpmatrix{W}}
\newcommand{\cbb}{\text{(c)}}

%\newcommand{\articleTitle}{Self-propulsion symmetries determine entropy production of active particles with hidden states}
\newcommand{\articleTitle}{Partial Entropy production of active particles with hidden states in potentials}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%% EPR with potential macros %%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\potential}[1]{V\left(#1\right)}
\newcommand{\potentialPrime}[1]{V'\left(#1\right)}
\newcommand{\potentialDoublePrime}[1]{V''\left(#1\right)}

\newcommand{\potentialx}{\potential{x}}
%\newcommand{\potentialxt}{V(x)|_{x(t)}}
\newcommand{\potentialxt}{\potential{x(t)}}
%\newcommand{\potentialxtn}[1]{V'(x)|_{x(t_{#1})}}
\newcommand{\potentialxtn}[1]{\potentialPrime{x(t_{#1})}}
%\newcommand{\potentialxtnShort}[1]{V'(x_{#1})}
\newcommand{\potentialxtnShort}[1]{\potentialPrime{x_{#1}}}

%\newcommand{\potentialxtzero}{V(x)|_{x(0)}}
\newcommand{\potentialxtzero}{\potential{x(0)}}
%\newcommand{\potentialxtT}{V(x)|_{x(T)}}
\newcommand{\potentialxtT}{\potential{x(T)}}
%\newcommand{\potentialxtR}{V(x)|_{x(T-t)}}
\newcommand{\potentialxtR}{\potential{x(T-t)}}
%\newcommand{\potentialprimex}{V'(x)}
\newcommand{\potentialprimex}{\potentialPrime{x}}
%\newcommand{\potentialprimext}{V'(x)|_{x(t)}}
\newcommand{\potentialprimext}{\potentialPrime{x(t)}}
%\newcommand{\potentialprimextR}{V'(x)|_{x(T-t)}}
\newcommand{\potentialprimextR}{\potentialPrime{x(T-t)}}
%\newcommand{\potentialdoubleprimex}{V''(x)}
\newcommand{\potentialdoubleprimex}{\potentialDoublePrime{x}}
%\newcommand{\potentialdoubleprimext}{V''(x)|_{x(t)}}
\newcommand{\potentialdoubleprimext}{\potentialDoublePrime{x(t)}}
%\newcommand{\potentialdoubleprimextR}{V''(x)|_{x(T-t)}}
\newcommand{\potentialdoubleprimextR}{\potentialDoublePrime{x(T-t)}}


\newcommand{\xplusVn}[1]{(\xdot(t_{#1})+\potentialxtn{#1})}
\newcommand{\xplusVnShort}[1]{(\xdot(t_{#1})+\potentialxtnShort{#1})}
\newcommand{\xplusVnShortR}[1]{(-\xdot(t_{#1})+\potentialxtnShort{#1})}
\newcommand{\xdotn}[1]{\xdot(t_{#1})}
\newcommand{\Cancel}[2][black]{{\color{#1}\cancel{\color{black}#2}}}
\newcommand{\DoubleCancel}[3]{{%
  \color{#1}\bcancel{\Cancel[#2]{#3}}%
}}

\newcommand{\CancelMan}[2][]{%
  \tikz[baseline=(X.base),inner sep=0pt]{%
    \node (X) {$#2$};
    \tikzset{#1}
    \draw[draw=#1, overlay, shorten >=-2pt, shorten <=-2pt] 
      (X.south west) -- (X.north east);
  }%
}
\newcommand{\DoubleCancelMan}[3]{%
  \tikz[baseline=(X.base),inner sep=0pt]{%
    \node (X) {$#3$};
    \draw[draw=#1, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=0pt]X.south west) -- ([xshift=-5pt]X.north east);
    \draw[draw=#2, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=5pt]X.south west) -- ([xshift=0pt]X.north east);
  }%
}
\newcommand{\TripleCancelMan}[4]{%
  \tikz[baseline=(X.base),inner sep=0pt]{%
    \node (X) {$#4$};
    \draw[draw=#1, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=4pt]X.south west) -- ([xshift=4pt]X.north east);
    \draw[draw=#2, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=0pt]X.south west) -- ([xshift=0pt]X.north east);
    \draw[draw=#3, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=-4pt]X.south west) -- ([xshift=-4pt]X.north east);
  }%
}

\newcommand{\bCancelMan}[2][]{%
  \tikz[baseline=(X.base),inner sep=0pt]{%
    \node (X) {$#2$};
    \tikzset{#1}
    \draw[draw=#1, overlay, shorten >=-2pt, shorten <=-2pt] 
      (X.north west) -- (X.south east);
  }%
}
\newcommand{\bDoubleCancelMan}[3]{%
  \tikz[baseline=(X.base),inner sep=0pt]{%
    \node (X) {$#3$};
    \draw[draw=#1, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=20pt]X.north west) -- ([xshift=0pt]X.south east);
    \draw[draw=#2, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=0pt]X.north west) -- ([xshift=-20pt]X.south east);
  }%
}
\newcommand{\bTripleCancelMan}[4]{%
  \tikz[baseline=(X.base),inner sep=0pt]{%
    \node (X) {$#4$};
    \draw[draw=#1, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=40pt]X.north west) -- ([xshift=0pt]X.south east);
    \draw[draw=#2, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=20pt]X.north west) -- ([xshift=-20pt]X.south east);
    \draw[draw=#3, line width=0.5pt, overlay, shorten >=-2pt, shorten <=-2pt]
      ([xshift=0pt]X.north west) -- ([xshift=-40pt]X.south east);
  }%
}

\newcommand{\subItem}[1]{
\begin{itemize}
\item{#1}
\end{itemize}
}

\newcommand{\triplePartial}[3]{
\partial_{t_#1}\partial_{t_#2}\partial_{t_#3}
}
\newcommand{\rmd}{\mathrm{d}}

\newcommand{\straightstraight}[4]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[Aactivity] (0.75,0) -- (-0.75,0) node [at start, above] {$_{#3},#4$} node [at end, above] {$_{#1},#2$};
    }
}
\newcommand{\straightstraightX}[5]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[Aactivity] (0.75,0) -- (-0.75,0) node [at start, above] {$_{#3},#4$} node [at end, above] {$_{#1},#2$} node [midway,below] {$#5$};
    }
}

\newcommand{\straightstraightdemoleft}[2]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[dotted] (0,0) -- (-0.75,0) node [at end, above] {};
    \draw[Aactivity] (0.75,0) -- (0,0) node [at start, above] {$_{#1},#2$};
    }
}

\newcommand{\straightstraightdemoright}[2]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[Aactivity] (0,0) -- (-0.75,0) node [at end, above] {$_{#1},#2$};
    \draw[dotted] (0.75,0) -- (0,0) node [at start, above] {};
    }
}

\newcommand{\wigglewiggle}[4]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[substrate] (0.75,0) -- (-0.75,0) node [at start, above] {$_{#3},#4$} node [at end, above] {$_{#1},#2$};
    }
}

\newcommand{\straightwiggle}[4]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[Aactivity] (0,0) -- (-0.75,0) node [at end, above] {$_{#1},#2$};
    \draw[substrate] (0.75,0) -- (0,0) node [at start, above] {$_{#3},#4$};
}
}

\newcommand{\wigglestraight}[4]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[substrate] (0,0) -- (-0.75,0) node [at end, above] {$_{#1},#2$};
    \draw[Aactivity] (0.75,0) -- (0,0) node [at start, above] {$_{#3},#4$};
}
}

\newcommand{\straightwigglestraight}[4]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[Aactivity] (-0.3,0) -- (-0.75,0) node [at end, above] {$_{#1},#2$};
    \draw[substrate] (0.3,0) -- (-0.3,0);
    \draw[Aactivity] (0.75,0) -- (0.3,0) node [at start, above] {$_{#3},#4$};
}
}

\newcommand{\wigglestraightwiggle}[4]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[substrate] (-0.3,0) -- (-0.75,0) node [at end, above] {$_{#1},#2$};
    \draw[Aactivity] (0.3,0) -- (-0.3,0);
    \draw[substrate] (0.75,0) -- (0.3,0) node [at start, above] {$_{#3},#4$};
}
}

\newcommand{\wigglestraightwigglestraight}[4]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[substrate] (-0.375,0) -- (-0.75,0) node [at end, above] {$_{#1},#2$};
    \draw[Aactivity] (0.0,0) -- (-0.375,0);
    \draw[substrate] (0.375,0) -- (0.0,0) ;
    \draw[Aactivity] (0.75,0) -- (0.375,0) node [at start, above] {$_{#3},#4$};
}
}

\newcommand{\straightwigglestraightwiggle}[4]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[Aactivity] (-0.375,0) -- (-0.75,0) node [at end, above] {$_{#1},#2$};
    \draw[substrate] (0.0,0) -- (-0.375,0);
    \draw[Aactivity] (0.375,0) -- (0.0,0) ;
    \draw[substrate] (0.75,0) -- (0.375,0) node [at start, above] {$_{#3},#4$};
}
}

\newcommand{\straightwigglestraightwigglestraight}[4]{
    \tikz[baseline=-2.5pt,scale=0.75]{
    \draw[Aactivity] (-0.45,0) -- (-0.75,0) node [at end, above] {$_{#1},#2$};
    \draw[substrate] (-0.15,0) -- (-0.45,0);
    \draw[Aactivity] (0.15,0) -- (-0.15,0) ;
    \draw[substrate] (0.45,0) -- (0.15,0) ;
    \draw[Aactivity] (0.75,0) -- (0.45,0) node [at start, above] {$_{#3},#4$};
}
}

%\newcommand{\tilderho}{\widetilde{\rho}}
\newcommand{\tildechi}{\widetilde{\chi}}

==> tikz_macros.tex <==
% \usepackage[colorlinks=true,linkcolor=black, urlcolor = black, citecolor = blue, anchorcolor = blue]{hyperref}

% \usepackage{graphicx}
% \usepackage[tight]{subfigure}
% \usepackage{multirow}
% \usepackage{subeqnarray}
% \usepackage{wasysym}
% \usepackage{eufrak}
% \usepackage{amsopn}


% \usepackage{amssymb}

% % For framed equations
% \usepackage{framed}

% % A4 papersize
% \usepackage{vmargin}
% \usepackage{epsfig}
% \usepackage{color}
% \usepackage{alltt}
% \usepackage{pstricks,pst-node,pst-tree,pst-grad,pst-text,graphics}
% \usepackage{dcolumn}
% \usepackage{url}

% % For an subcases math env
% \usepackage{cases}

% % For backreferences in the bibliography
% %\usepackage{backrefx}

% % For proper presentation of references
% %\usepackage{natbib}
% %\usepackage[square,numbers]{natbib}
% %\bibliographystyle{unsrt}
% %\newcommand{\posscitet}[1]{\citeauthor{#1}'s (\citeyear{#1})}

% % Used in a macro
% \usepackage{ifthen}

% % For flushing figures after current page has finished
% \usepackage{afterpage}

% % To comment out large chunks
% \usepackage{comment}

% % For extra long table
% \usepackage{supertabular}

% % To have or have not space after abbreviations (used in some
% % ``macros'')
% \usepackage{xspace}

% % For the spaing used below
% \usepackage{setspace}

% % For nicer captions
% \usepackage[bf,footnotesize]{caption}

% % For marginal notes as floats (actually only for having a table of them)
% %\usepackage{float}

% % For legal symbols (\textregistered etc.)
% \usepackage{textcomp}

% For diagrams in second_quantisation.tex
\usepackage{tikz}
\usetikzlibrary{decorations.pathmorphing}
\usetikzlibrary{decorations.markings}
\usetikzlibrary{arrows,shapes,snakes,automata,backgrounds,petri}
\usetikzlibrary{calc}
\usetikzlibrary{patterns}
\usetikzlibrary{decorations.text}
% The t-styles are for text, the A-styles are amputated, the S-style
% have shifted arrow.
\tikzset{
xxtsubstrate/.style={decorate, 
line width=1pt,
draw=olive, 
decoration=snake, 
%segment amplitude=0.5mm, 
%segment length=5pt,
segment amplitude=0.75mm, 
line after snake=0.25mm,
line before snake=0.25mm
},
tsubstrate/.style={decorate, 
line width=1pt,
draw=olive, 
decoration=snake, 
segment amplitude=0.5mm, 
segment length=5pt,
segment amplitude=0.2mm, 
line after snake=1mm,
line before snake=1mm
},
Bsubstrate/.style={decorate, 
line width=1pt,
draw=orange, 
%decoration=coil,
decoration=snake,
segment length=5pt,
segment aspect=0,
segment amplitude=0.5mm, 
line after snake=0mm,
line before snake=0mm
},
substrate/.style={decorate, 
line width=1pt,
draw=orange,%olive, 
%snake=snake, 
decoration=snake, 
%segment amplitude=0.5mm, 
segment length=5pt,
segment amplitude=0.5mm, 
line after snake=0.5mm,
line before snake=0.5mm
},
activity/.style={very thick,draw=red,postaction={decorate},
decoration={markings,mark=at position .5 with
{\arrow[draw=red]{>}}}},
tactivity/.style={thick,draw=red,postaction={decorate},
decoration={markings,mark=at position .5 with
{\arrow[draw=red]{>}}}},
tEPSactivity/.style={thick,draw=red,postaction={decorate},
decoration={markings,mark=at position .55 with
{\arrow[draw=red]{>}}}},
tAactivity/.style={thick,draw=red},
Aactivity/.style={thick,draw=black},
tSactivity/.style={thick,draw=red,postaction={decorate},
decoration={markings,mark=at position .7 with
{\arrow[draw=red]{>}}}},
Sactivity/.style={very thick,draw=red,postaction={decorate},
decoration={markings,mark=at position .7 with
{\arrow[draw=red]{>}}}},
polarity/.style={decorate, 
line width=1pt,
draw=black,%olive, 
%decoration=border, 
decoration={markings,mark=between positions 0 and 1 step 1.6mm with {\draw[black,thick,fill=black]  (0,0) circle (0.02)} },
%segment amplitude=0.5mm, 
segment length=5pt,
segment amplitude=0.5mm, 
%line after markings=0.5mm,
%line before markings=0.5mm
},
Bpolarity/.style={decorate, 
line width=1.5pt,
draw=red,
%densely dashed,
segment length=5pt,
segment amplitude=0.5mm, 
%line after markings=0.5mm,
%line before markings=0.5mm
},
density/.style={ 
line width=1.5pt,
draw=magenta,
densely dashed,
segment length=5pt,
segment amplitude=0.5mm, 
%line after markings=0.5mm,
%line before markings=0.5mm
},
%alphatbeta/.style={decorate,
%decoration={decoration={markings,mark=between positions 0 and 1 step 1.5mm with {\draw[red,thick]  (0,0) circle (0.04)} },pre={draw=black,densely dashed,},pre length=5pt},
%}
}

\newcommand{\crossblob}[2][]{\coordinate (a) at (#2);
\draw[color=olive,line width=1pt,fill=white,text=black,outer sep=2pt] (a) circle (0.15cm) node [above] {#1};%
\draw[color=olive,line width=1pt] ($  (45:0.15cm) + (a) $) -- ($ (45:-0.15cm) + (a) $);%
\draw[color=olive,line width=1pt] ($ (-45:0.15cm) + (a) $) -- ($ (-45:-0.15cm) + (a) $);%
}

% https://tex.stackexchange.com/questions/473321/tikz-custom-dotted-pattern
\pgfdeclarepatternformonly{densedots}{\pgfqpoint{-1pt}{-1pt}}{\pgfqpoint{1pt}{1pt}}{\pgfqpoint{2pt}{2pt}}% original definition: \pgfqpoint{3pt}{3pt}
{%
  \pgfpathcircle{\pgfqpoint{0pt}{0pt}}{.5pt}%
  \pgfusepath{fill}%
}%


\newcommand{\fourPointConnectedA}[4]{
\tikz[baseline=-2.5pt]{
      \draw[Aactivity] (0,0.0) -- (0.25,0.0) +(2pt,0) circle (2pt)[fill];
      \begin{scope}[rotate=0]
      \draw[Aactivity] (220:0.7) -- (0,0.0);
      \draw[dotted,thin] (140:0.25) arc (140:220:0.25); 
      \draw[Aactivity] ($(-0.07,0.07)+(220:0.2)$) -- ($(0.07,-0.07)+(220:0.2)$);
      \end{scope}
      \draw[Aactivity] (140:0.7) -- (0,0.0);
      \draw[Aactivity] ($(0.07,0.07)+(140:0.2)$) -- ($(-0.07,-0.07)+(140:0.2)$);
      \begin{scope}[xshift=-0.54cm,yshift=0.45cm]
      \draw[Aactivity] (220:0.6) -- (0,0.0);
      \draw[Aactivity] (140:0.6) -- (0,0.0);
      \draw[dotted,thin] (140:0.25) arc (140:220:0.25);
      \draw[Aactivity] ($(0.07,0.07)+(140:0.2)$) -- ($(-0.07,-0.07)+(140:0.2)$);
      \draw[Aactivity] ($(-0.07,0.07)+(220:0.2)$) -- ($(0.07,-0.07)+(220:0.2)$);
     \end{scope}
     \begin{scope}[xshift=-0.54cm,yshift=-0.45cm]
      \draw[Aactivity] (220:0.6) -- (0,0.0);
      \draw[Aactivity] (140:0.6) -- (0,0.0);
      \draw[dotted,thin] (140:0.25) arc (140:220:0.25);
      \draw[Aactivity] ($(0.07,0.07)+(140:0.2)$) -- ($(-0.07,-0.07)+(140:0.2)$);
      \draw[Aactivity] ($(-0.07,0.07)+(220:0.2)$) -- ($(0.07,-0.07)+(220:0.2)$);
     \end{scope}
    \node [yshift=0.8cm,xshift=-1.2cm] {$#1$};
    \node [yshift=0.25cm,xshift=-1.2cm] {$#2$};
    \node [yshift=-0.15cm,xshift=-1.2cm] {$#3$};
    \node [yshift=-0.8cm,xshift=-1.2cm] {$#4$};
    }
}

\newcommand{\fourPointConnectedB}[4]{
\tikz[baseline=-2.5pt]{
      \begin{scope}[rotate=0]
      \draw[Aactivity] (220:1) -- (0,0.0);
      \draw[Aactivity] ($(-0.07,0.07)+(220:0.2)$) -- ($(0.07,-0.07)+(220:0.2)$);
      \end{scope}
      \draw[Aactivity] (140:0.5) -- (0,0.0);
      \draw[Aactivity] ($(0.07,0.07)+(140:0.2)$) -- ($(-0.07,-0.07)+(140:0.2)$);
      \draw[dotted,thin] (140:0.25) arc (140:220:0.25);
      \begin{scope}[xshift=-0.35cm,yshift=0.3cm]
      \draw[Aactivity] (220:0.6) -- (0,0.0);
      \draw[Aactivity] (140:0.6) -- (0,0.0);
      \draw[Aactivity] ($(0.07,0.07)+(140:0.2)$) -- ($(-0.07,-0.07)+(140:0.2)$);
      \draw[Aactivity] ($(-0.07,0.07)+(220:0.2)$) -- ($(0.07,-0.07)+(220:0.2)$);
      \draw[dotted,thin] (140:0.25) arc (140:220:0.25);
     \end{scope}
     \begin{scope}[xshift=0.45cm,yshift=-0.38cm]
      \draw[Aactivity] (220:0.8) -- (0,0.0);
      \draw[Aactivity] (140:0.6) -- (0,0.0);
      \draw[Aactivity] (0,0.0) -- (0.4,0.0) +(2pt,0) circle (2pt)[fill];
      \draw[Aactivity] ($(0.07,0.07)+(140:0.2)$) -- ($(-0.07,-0.07)+(140:0.2)$);
      \draw[Aactivity] ($(-0.07,0.07)+(220:0.2)$) -- ($(0.07,-0.07)+(220:0.2)$);
      \draw[dotted,thin] (140:0.25) arc (140:220:0.25);
     \end{scope}
    \node [yshift=0.8cm,xshift=-1.cm] {$#1$};
    \node [yshift=0.1cm,xshift=-1.cm] {$#2$};
    \node [yshift=-0.5cm,xshift=-1.cm] {$#3$};
    \node [yshift=-0.9cm,xshift=-0.4cm] {$#4$};
    }
}
